Longitudinal change in language behaviour during protests: A case study of Euromaidan in Ukraine

In the last decade, online social media has become the primary platform for protesters to organize and express their agenda in various parts of the world. Nevertheless, scholars still debate whether online tools induce offline protests or facilitate them. Unfortunately, studies of protests often lack panel data and cannot address how particular users change their behaviour over time in line with the protest agenda. To this end, we analyze a new dataset of the Facebook page EuroMaydan that was explicitly created to facilitate the protest in Ukraine from November 2013 to February 2014. Moreover, our analysis follows this page even after the end of the protest till June 2014. In total, the dataset includes 26,631 posts and 1,470,593 comments that were generated by 124,790 users during and after the protests. We use this panel data to test how particular users switch between the two most popular languages of this page: Ukrainian and Russian. Previous studies have puzzled with language behaviour during the Ukrainian protest. Although researchers expected to see more Ukrainian language due to national mobilization, studies discovered that Ukrainian protesters frequently used Russian, especially after the end of the protest. A hypothesis was suggested that protesters use language strategically depending on circumstances (e.g., to maximize outreach). However, previous studies relied on aggregated data and did not explore the within-subject variation of language behaviour. Our study adds to this scholarship by adding a longitudinal analysis of language behaviour. Considering the broader contribution of this paper, we add to the literature on protests by validating previous findings derived from surveys that activists change their behaviour to reflect prior preferences and situational goals rather than modify their preferences.

==> Do_past.tex <==
\section{Did people change their language usage behaviour in social media?}
\label{sec:Language switching patterns}
Our analysis begins with understanding whether it is possible to find evidence that some of the users changed their language usage behaviour. \fixme{The whole analysis is about Euromaiden so not sure what is the point of this line?} At the same time, we also assume that this change couldn't happen randomly but possibly was triggered by some major external events, such as the Euromaidan revolution that significantly influenced the self-identification of Ukrainians. To be more specific, we concentrate on the comments of the users and check whether the users start to prefer the Russian or Ukrainian language more after the revolution than they used before. 

By so doing, we want to see if the general trends of some individual's \fixme{are we sure we are doing individual?} language behaviour changed over time. Then, in what follows, we will zoom in to the desegregated data of \fixme{particular is a strong word here. Have we anaylysed any particular users?} particular individuals and analyze the within-subject variation.

\subsection{Data selection and preprocessing}
We start with a brief description of the data preparation pipeline. The pipeline consists of the three steps: comment text preprocessing, comment language classification and active user identification. Below, a more detailed description of each of the steps that are discussed.

\subsubsection{1) Text preprocessing:}
We preprocessed raw comments using a standard text preprocessing pipeline: lowercase the text, remove punctuation, URLs and numbers.
    
\subsubsection{2) Comment language classification:}
To identify the language of the comment, we use a text language classification model from FastText\footnote{\url{https://fasttext.cc/}}. For the reliable results of the analysis, this model must be accurate enough on our data. To verify this, we calculate the accuracy of the model on a sample of 2000 random comments from our dataset. We manually label each of the comments from the sample and then compare the label with the models' prediction. 
It turns out that the accuracy is 96\% for the language classification task, which is considered good, and thus we continue our analysis. Based on the language prediction, out of all the comments, 59\% of them are in Russian, 31\% in Ukrainian, and 10\% are comments in other languages. We then exclude comments in languages other than Russian and Ukrainian, due to their marginal presences, and in addition they are beyond the scope of our research question. 

\fixme{The following para is very technical details. It appears as if we are describing the algorithm/approah but it is not needed? I will come to this again}
Then we create a new column called \textit{comment\_language} where we create a label \textbf{1} if a comment text is in Ukrainian language and \textbf{0} if the comment text is in Russian. Finally, we sort comments by the date published (\textit{comment\_published}) and group \textit{comment\_language} at the level of user (\textit{comment\_by}). In the end, we receive a binary language vector for each of the users

\subsubsection{3) Active users identification}
In what follows, we will discuss the approach of language preference detection. This approach requires a sufficient number of comments per user. Otherwise, the analysis can be harmed by spurious effects due to a lack of data. As Figure \ref{figure:number_of_comments_histogram} shows that most of the users in our dataset are not active and commented only a few times. More precisely, the mean number of comments per user is 12, while the second (median) and third quartile are 2 and 7, respectively. Therefore, to select only relevant users that can provide us reliable results, we fix a \textit{threshold} by the number of their comments. We call the users with at least \textit{threshold} number of comments as active users, and the way we choose \textit{threshold} is described later in Section \ref{subsection: language change identification}. 

%In the approach of language preference detection, which we discuss later, we will use the language binary vectors of the users. The number of comments of the users we analyze must be high enough to avoid spurious effects due to a lack of data. 

\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{Images/number_of_user_comments.pdf}
\caption{Histogram of the number of comments per user}
\label{figure:number_of_comments_histogram}
\end{figure}

\subsection{The identification of the change of the language usage behaviour}
\label{subsection: language change identification}

% We begin this session by running a statistical test comparing two proportions of the comments in Ukrainian language before and the end of the revolution.

% We use statistical methods to prove that there was indeed a change in the language usage of a given user. In particular, we use hypothesis testing about two proportions. To split the language vector of the user into two sub-vectors (to calculate proportions then), we select a specific date as a separator. The date we select for this role is the date of the end of the Euromaidan revolution. Below is a more detailed description of this approach.

We use statistical methods about comparing two proportions to prove that there was indeed a change in the language usage of a given user. The null hypothesis is \textit{P1} - \textit{P2} $\geq$ 0, and the alternative hypothesis is \textit{P1} - \textit{P2} $<$ 0, where \textit{P1} is the proportion of the comments in the Ukrainian language before the end of the revolution and \textit{P2} is also a proportion of comments in Ukrainian language but after the revolution. \fixme{Expain why do we choose exactly one sided hypothesis}. In the same manner, we also compare the proportions of Russian comments before and after the end of Euromaidan. 

% This is the first step in our analysis. By so doing, we want to see if the general trends of some individual's language behaviour changed over time. Then, in what follows, we will zoom in to the desegregated data of particular individuals and analyze the within-subject variation.

%In such a way, if we statistically find that the difference between two proportions is significant, that can indicate that the user changed his or her behaviour.

% As we described previously, it is important to select active users for the analysis using a specific threshold by the number of comments to receive reliable results. Agresti and Franklin (2007) (\fixme{Insert a valid reference}) have suggested a rule of thumb for its minimum sample size that there should be at least ten successes and ten failures in each sample. Therefore, we start with selecting users with at least ten comments in one and ten comments in another sample (so at least 20 comments, which is approximately 90 quantile for us). \fixme{Raj@Ivan: This paragraph is not very clear to me.}

As described previously, it is important to select active users with sufficient comments to receive reliable results from statistical tests about the difference between the two proportions. To find this threshold by the number of comments, we follow the suggestion from Agresti and Franklin (2007) \fixme{Insert a valid reference}. The authors propose a rule of thumb for its minimum sample size: at least ten successes and ten failures in each sample. In our case, it means that the user should have at least ten comments in the Russian language and ten comments in the Ukrainian language in one sample (before the split date) and another (after the split date.). \fixme{Why end of revolution is selected as a date to compare the proportions?}


\subsubsection{Robustness check}
We also execute robustness checks to make sure that our findings are stable across different thresholds. To this end, we marginally increase our requirement to the minimal sample size in several steps (see Table \ref{table:Stable thresholds} for more detailed thresholds). Furthermore, we vary our split date which indicates the end of the protest. We also try a date one month before and one month after the initial date we chose. We expect to observe, that the number of rejections of the null hypothesis should be lower than, if we choose exactly the date of Euromaindan for split. 

Finally, we calculate the number of rejections of the null hypothesis for each of the active users. In all the cases, we use a significance level of 0.05. The results for Russian and Ukrainian languages can be found in Table \ref{table:Russian results} and \ref{table:Ukrainian results}, respectively. 


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\textbf{Number of users} & \textbf{Positive threshold} & \textbf{Negatives threshold} \\ \hline
              557                  & 10                                & 10                                \\ \hline
              313                 & 15                                & 15                                \\ \hline
              192                 & 20                                & 20                                \\ \hline
\end{tabular}%
}
\caption{Thresholds of each sample for active users selection}
\label{table:Stable thresholds}
\end{table}

% Finally, we calculate the number of rejections of the null hypothesis for each of the active users. In all the cases, we use a significance level of 0.05. The results for Russian and Ukrainian languages can be found in Table \
% \begin{enumerate}
%     \item \textbf{With threshold 10:}, 46\% of active users started to use Russian more frequently, while only 4\% started to use Ukrainian more frequent.
%     \item \textbf{With threshold 15:}, 53\% of active users started to use Russian more frequently, while only 3\% started to use Ukrainian more frequent.
%     \item \textbf{With threshold 20:}, 57\% of active users started to use Russian more frequently, while only 3\% started to use Ukrainian more frequent.
% \end{enumerate}


\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{}           & \textbf{22 Jan 2014} & \textbf{22 Feb 2014} & \textbf{22 Apr 2014} \\ \hline
\textbf{Threshold: 10} &  4\%              &    4\%              &  3\%              \\ \hline
\textbf{Threshold: 15} &  2\%               &    3\%              &   2\%              \\ \hline
\textbf{Threshold: 20} &  2\%                &    3\%              &    2\%            \\ \hline
\end{tabular}%
}
\caption{Ukrainian language proportion test results}
\label{table:Ukrainian results}
\end{table}


\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{}           & \textbf{22 Jan 2014} & \textbf{22 Feb 2014} & \textbf{22 Apr 2014} \\ \hline
\textbf{Threshold: 10} & 40\%                &  46\%               &  44\%              \\ \hline
\textbf{Threshold: 15} & 45\%               &  53\%            & 51\%               \\ \hline
\textbf{Threshold: 20} &  50\%                 &  57\%               & 53\%               \\ \hline
\end{tabular}%
}
\caption{Russian language proportion test results}
\label{table:Russian results}
\end{table}


\fixme{COMMENT FROM IVAN: I WILL COME BACK TO IT LITTLE BIT LATER TO MATCH THE SECTIONS BETTER }

\fixme{Tym @all: i think some conclusion must be here. We show tables, but what to we want to say? 2 percent in Table 3 and 57 percent in Table 4 -- what do they mean}\textcolor{blue}{Raj@Tym: I agree with you.}

\fixme{Tym@all: i think now we have to add 4.3. IS ONE LANGUAGE IS MORE STICKY THAN OTHER. And say something like this. We established that on average people change languages in XXXX cases. Now we can elaborate our finding and analyze the withing-subject variation. In other words, we will investigate individual trajectories and how people changed their behavior over time. To this end we compare whether languages are sticky. We will analyze what was the typical pattern for individuals. For instance, some people adapted new language and used it consistently, while other people were jumping from one language to another depending on circumstances. COPE PASTE section 5.3. here and make it 4.3.} \textcolor{blue}{Raj@Tym: but there is no section 5.3. If you meant 5.1?}


% \subsection{Is one language is more sticky than other?}
% \fixme{title suggestion: If the stickiness is same across both the languages?}
% % By now, we provide two hypotheses about why a given user may change his behaviour. At the same time, we don't investigate why there is a significant difference between the preference increase in Russian and Ukrainian languages.  

% In this part of the analysis, we investigate the moment of the language in the sequence of the user's comments ordered by time. Therefore, we transform them again using the following procedure: if the next comment language is the same as the previous one, we put \textbf{0}, otherwise \textbf{1}. After that, we analyze the normalized frequencies of such changes and the lengths of the longest sequences without switches. Our main aim is to compare Russian and Ukrainian users and whether their behaviour is similar or not. We provide more details later in this section.
% We start our analysis with the investigation of how frequently users switched from one language into another. 
% The cumulative frequency of this measure is illustrated in Figure \ref{figure:language_change_frequency}. It can be noted that 43\% of users rarely changed their language, i.e. they switched their language in between of 0\% to 10\% of their comments. 

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{Images/language_frequency.pdf}
% \caption{Language change frequency \fixme{why not cumulative plot, using lineplot?}}
% \label{figure:language_change_frequency}
% \end{figure}

% Figure  \ref{figure:consequtive_language} shows the normalized length of the longest sequence of user comments in the same language. It shows that a significant amount of users always stayed with the same language (right side of the graph). At the same time, most of the users switched somewhere in between of 20\% to 40\% of their comments.  

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{Images/ll_usage.pdf}
% \caption{Longest consecutive usage of the same language}
% \label{figure:consequtive_language}
% \end{figure}

% The comparison between the Russian and Ukrainian language users is presented in the Figure \ref{plot:longest-usage-ru-uk}. 
% We define language users if they use a particular language at least 80\% \fixme{why this number?, we need to provide justification} of times among all comments. 

% \begin{figure}[!h]
% \centering
% \includegraphics[width=\columnwidth]{Images/RuAndUaMeanLanguages.pdf}
% \caption{Mean language histogram}
% \label{figure:russian_ukrainian}
% \end{figure}

% Then we compare cumulative language frequency for Facebook-Russian-speakers (Figure \ref{plot:longest-usage-ru-uk} (a)) and Facebook-Ukrainian-speakers (Figure \ref{plot:longest-usage-ru-uk} (b)). These figures show a remarkable difference between the Russian-speakers and Ukrainian-speakers users. Russian-speakers users do not change their language behavior in 69\% of comments, whereas Ukrainian-speakers users do not change their behavior in only 16\% comments. To put it simply, the Ukrainian-speakers are more flexible. They use Ukrainian language once and then they change it to Russian and then they go back to Ukrainian.  

% This trend is even more pronounced in Figure \ref{plot:cumulative-russian-ukrainian}. They show the longest consecutive usage of the language by Russian-speakers users and Ukrainian-speakers users. Again, most of the Russian-speakers users stick to one language and rarely change it, whereas most of the Ukrainian-speakers users switch from one language to another in 30\% to 40\% of their activities. 

% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/ll_usage_ru.pdf}} 
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/ll_usage_ua.pdf}} 
%     \caption{Longest consecutive usage of the Russian and Ukrainian language}
%     \label{plot:longest-usage-ru-uk}
% \end{figure*}


% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/language_frequency_russians.pdf}}
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/language_frequency_ukrainians.pdf}}
%     \caption{Cumulative language change frequency for the Russian and Ukrainian language}
%     \label{plot:cumulative-russian-ukrainian}
% \end{figure*}

% This observation tells us that the Russian language is stickier than the Ukrainian language. Meaning that users who prefer Russian are not prone to change their minds and switch to another language. In comparison, the Ukrainian language users are more flexible, thus showing much lower language preference change when we perform hypothesis testing. 






% \begin{figure*}[h]
% 	%\vspace{-10pt}
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/UpdatedPlots/ll_usage_ru.pdf}
% 		\label{plot:longest-usage-ru}
% 	}~\hfill
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/UpdatedPlots/ll_usage_ua.pdf}
% 		\label{plot:longest-usage-uk}
% 	}
%  \caption{Longest consecutive usage of the Russian and the Ukrainian language users}
%   \label{plot:longest-usage-ru-uk}
% \end{figure*}

% \begin{figure*}[t]
% 	%\vspace{-10pt}
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/ll_usage_ru.pdf}
% 		\label{plot:longest-usage-ru}
% 	}~\hfill
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/ll_usage_ua.pdf}
% 		\label{plot:longest-usage-uk}
% 	}
%  \caption{Longest consecutive usage of the Russian and Ukrainian language\fixme{Font of X and Y axis is too small}}
%   \label{plot:longest-usage-ru-uk}
% \end{figure*}









% \fixme{Raj@Ivan: What is the definition of active users in this and local section? If I remember the active users definition changes in section 5.1}
% % By now, we provide two hypotheses about why a given user may change his behaviour. At the same time, we don't investigate why there is a significant difference between the preference increase in Russian and Ukrainian languages.  

% In previous sections we investigated the role of posts and new users \fixme{it should be reverse?}. However, we also would like to see if the choice of the language is stable. %In this part of the analysis, we investigate the moment of the language in the sequence of the user's comments ordered by time. 

% To investigate this question, we firstly reorganize our data in the following way: \fixme{I think we should start with the posts? - For each post or for each user? For each user we created a language vector.} if the next comment language is the same as the previous one, we put \textbf{0}, otherwise \textbf{1}. After that, we analyze the normalized frequencies of such changes and the lengths of the longest sequences without switches. Our main aim is to compare active users who are known to use primarily Russian and Ukrainian languages. We start our analysis with the investigation of how frequently users switched from one language into another. 

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{Images/language_frequency.pdf}
% \caption{Language change frequency \fixme{why not cumulative plot, using lineplot?}}
% \label{figure:language_change_frequency}
% \end{figure}

% \fixme{Raj@Ivan:Till this point, we have not pointed to Figures 3, 4, 5 and 6?}

% Figure  \ref{figure:consequtive_language} shows the normalized length of the longest sequence of user comments in the same language. It shows that a significant amount of users always stayed with the same language (right side of the graph). At the same time, most of the users switched somewhere in between of 20\% to 40\% of their comments.  

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{Images/ll_usage.pdf}
% \caption{Longest consecutive usage of the same language}
% \label{figure:consequtive_language}
% \end{figure}

% \fixme{No reference to Figure 8 and suddenly we are discussing Figure 9 next?}
% The comparison between the Russian and Ukrainian language users is presented in the Figure \ref{plot:longest-usage-ru-uk}. 
% We define language users if they use a particular language at least 80\% \fixme{why this number?, we need to provide justification} of times among all comments. 

% \begin{figure}[!h]
% \centering
% \includegraphics[width=\columnwidth]{Images/RuAndUaMeanLanguages.pdf}
% \caption{Mean language histogram}
% \label{figure:russian_ukrainian}
% \end{figure}

% Then we compare cumulative language frequency for Facebook-Russian-speakers (Figure \ref{plot:longest-usage-ru-uk} (a)) and Facebook-Ukrainian-speakers (Figure \ref{plot:longest-usage-ru-uk} (b)). These figures show a remarkable difference between the Russian-speakers and Ukrainian-speakers users. Russian-speakers users do not change their language behavior in 69\% of comments, whereas Ukrainian-speakers users do not change their behavior in only 16\% comments. To put it simply, the Ukrainian-speakers are more flexible. They use Ukrainian language once and then they change it to Russian and then they go back to Ukrainian.  

% This trend is even more pronounced in Figure \ref{plot:cumulative-russian-ukrainian}. They show the longest consecutive usage of the language by Russian-speakers users and Ukrainian-speakers users. Again, most of the Russian-speakers users stick to one language and rarely change it, whereas most of the Ukrainian-speakers users switch from one language to another in 30\% to 40\% of their activities.


% \begin{figure*}[t]
% 	%\vspace{-10pt}
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/ll_usage_ru.pdf}
% 		\label{plot:longest-usage-ru}
% 	}~\hfill
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/ll_usage_ua.pdf}
% 		\label{plot:longest-usage-uk}
% 	}
%  \caption{Longest consecutive usage of the Russian and Ukrainian language\fixme{Font of X and Y axis is too small}}
%   \label{plot:longest-usage-ru-uk}
% \end{figure*}


% \begin{comment}
% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/ll_usage_ru.pdf}} 
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/ll_usage_ua.pdf}} 
%     \caption{Longest consecutive usage of the Russian and Ukrainian language}
%     \label{plot:longest-usage-ru-uk}
% \end{figure*}
% \end{comment}


% \begin{figure*}[t]
% 	%\vspace{-10pt}
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/language_frequency_russians.pdf}
% 		\label{plot:cumulative-russian}
% 	}~\hfill
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/language_frequency_ukrainians.pdf}
% 		\label{plot:cumulative-ukrainian}
% 	}
% \caption{Cumulative language change frequency for the Russian and Ukrainian language\fixme{Font of X and Y axis is too small}}
%     \label{plot:cumulative-russian-ukrainian}
% \end{figure*}

% \begin{comment}
% \begin{figure*}[!h]
%     \centering
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/language_frequency_russians.pdf}}
%     \subfigure[]{\includegraphics[width=0.45\textwidth]{Images/language_frequency_ukrainians.pdf}}
%     \caption{Cumulative language change frequency for the Russian and Ukrainian language}
%     \label{plot:cumulative-russian-ukrainian}
% \end{figure*}
% \end{comment}


%This observation tells us that the Russian language is stickier than the Ukrainian language. Meaning that users who prefer Russian are not prone to change their minds and switch to another language. In comparison, the Ukrainian language users are more flexible, thus showing much lower language preference change when we perform hypothesis testing.


% \fixme{By Tym. Note about the language of the post. We know that the posts are made by managers of the page. So it does not really matter. They post in Russian or Ukrainian, but they always post somethig GOOD about Euromaidan. So I would do here 2 things:

%In the current section, we continue our analysis of such a phenomenon. In particular, we will try to formulate hypotheses of what has potentially influenced the active users' language choice in comments and provide a possible explanation. 

%We need to emphasize that the reasons for behaviour change can be more than our data allows us to spot and prove. This is one of the limitations of our study and available data to investigate (more about limitations in Section \ref{chapter:limitations}).

% \subsection{Do the group shape the language preference of the active users? (Global influence)}
% We start with a hypothesis that the language preferences in the group can shape the individual user's preferences. Meaning, the more a given user observe a particular language's prevalence in a large group (or in a global context), the more this user starts to use this language in his or her own conversations. 

% To give some evidence of the possibility of such a hypothesis, we can start with the observation that the number of Russian comments is the largest in our dataset (see Section \ref{sec:Language switching patterns}). However, the interesting observation here is that the number of Russian and Ukrainian comments was approximately the same before February 2014 (the month in which Euromaidan ended). Figure \ref{figure:russian_and_ukrainian} shows this observation more in detail. 

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{Images/RussianAndUkrainian.pdf}
% \caption{Number of comments in Russian and Ukrainian language}
% \label{figure:russian_and_ukrainian}
% \end{figure}

% %NEW TEXT
% Our data also allows us to test whether the post itself has any impact on the language of the comment. We use Pearson's correlation coefficient to calculate if the language of the post correlates with the language of the comments. The correlation coefficient between the post and comment language for the general population of users is only 0.13, which indicates a very week relationship. This observation shows that users who leave comments do not mind the post language agenda. In other words, users will keep using Ukrainian language even if the post is in Russian and vice versa. This observation suggests that it is not easy to manipulate and nudge language behavior of people. 

% We could find one possible explanation of such behaviour if we look at the plot of the appearances of the new users in the group on Figure \ref{figure:new_users}. Here, we define new users as users who made their first comment on a given date. The figure partially explains this trend by showing the influx of new users in the group. Some of them were likely to be people who joined the Facebook page after the end of the protest to follow the political agenda, and others were existing users who were likely to be silent during the protest. We do not know the exact reason. However, we assume that three possible explanations for why silent users became active after the end of Euromaidan. First, it is possible that people were busy following the logistics of the protest agenda, and they did not have time or need to discuss political news. After the protest, these people are no longer involved in the logistics, and they can debate political news. Another possible explanation is the influx of bots or Russian (or pro-Russian) activists who could enter this group to shape its content, respectively \cite{metzger2016tweeting}. Finally, it is possible that some users used Russian strategically to convey their agenda to their respective audiences.

% \begin{figure}[h]
% \centering
% \includegraphics[width=\columnwidth]{Images/new_users.pdf}
% \caption{The appearances of the new users}
% \label{figure:new_users}
% \end{figure}


% \begin{figure*}[h!]
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/UpdatedPlots/language_frequency_russians.pdf}
% 		\label{plot:cumulative-russian}
% 	}~\hfill
% 	\subfloat[]{
% 		\includegraphics[width=0.45\textwidth]{Images/UpdatedPlots/language_frequency_ukrainians.pdf}
% 		\label{plot:cumulative-ukrainian}
% 	}
% \caption{Cumulative language change frequency for the Russian and the Ukrainian language users among \textit{active users}}
%     \label{plot:cumulative-russian-ukrainian}
% \end{figure*}

==> Ukrainian_context.tex <==
% \section{Ukrainian context}
% \label{sec:Ukrainian context}

%Survey data have shown that during the transition period of the 1990s and early 2000s Ukrainians rarely trusted to formal institutions and rarely engaged in informal relationship (Gatskova and Gatskov 2020). Moreover, some studies prior to the EuroMaydan Revolution argued that “informal relationships arise exclusively between individuals who personally trust each other and therefore the interactions may occur between acquaintance of acquaintance but not with the persons not directly known by the circle of trusted persons” (Gatskova & Gatkskov, 2012, p. 26). Thus, the EuroMaidan revolution hit many as a surprising and unexpected since it grew up from a set of grass-rooted mass protest in the end of November 2013. This revolution relayed on various volunteering organizations that mushroomed in Kyiv in order to provide supplies, food, defense, psychological support, legal advice, medical care (including mobile surgical hospitals), information and analytical overviews etc. With time, this revolution influenced a development of new volunteering movements and civil society organizations. EuroMaidan has received a significant attention among researchers. Most of the scholars addressed political and national mobilization as well as nationalist narratives of the revolution (Chayinska et al. 2019; Gladun 2020; Onuch 2014; Onuch and Sasse 2016; Zhuravlev and Ishchenko 2020). Other papers addressed consequential events of the Crimea annexation and hybrid war with Russia (Giuliano 2018; Kudelia and van Zyl 2019; Sasse and Lackner 2018; Zolkina and Haran 2017). Sociologists and economists focused on the consequences of Euromaidan for national solidarity, economic development, and wellbeing in regions (Ivaschenko-Stadnik 2020; Sereda 2020; Coupe and Obrizan 2016(a); Coupe and Obrizan 2016(b); Vakhitova and Iavorskyi 2020; Zhukov 2016). Considering the progress of the revolution, a polling company “Democratic initiative foundation” conducted three surveys during the revolution. Researchers from this organization classified three periods of the revolution by the stages of organization: “Protest”, “Camp” and “Sich” (the last title is a reference to the quasi state of Ukrainian Cossacks). According to the survey data, this was a protest of mainly men in their 30-54; the majority of protesters had higher education degree; a significant share of them arrived to the capital from other regions. 
%A group of independent researchers conducted another survey in two Ukrainians cities Lviv and Kyiv during the Euromaidan (Shestakovskiy, 2014). The goal of this survey was to analyze the structure of values of social activists employing the Swartz scheme of values. Sviatnenko & Vinogradov (2014) used these data documenting that Ukrainians who participated in the revolution had higher values of Universalism and Self-Direction compared to the national sample of Ukrainians surveyed before. Some other researchers investigated the everyday life of protesters with emphasis on the gender roles, task division among volunteers, identities of activists, right-wing participation (Ishchenko, 2014; Juravlev, 2014; Onuch & Martsenyuk, 2014; Popova, 2014; Phillips, 2014; Stepurko et.al, 2014;).
%A study of Onuch (2015) is an important contribution to the analysis of the role of Internet in EuroMaidan developments. As she indicates, Facebook (among other online social networks) was not the central mechanism of the mobilization.  However, network connectivity among protesters was facilitated greatly by online social networks. Some other studies of online activities during the revolution addressed how protesters used Twitter, Facebook, and Vkontakte (Jost et al. 2018; Tucker et al. 2014; Gruzd and Kampen 2016; Metzger et al. 2016). These studies show that OSM were instrumental in providing logistical support for protesters. Particularly, Jost et al. (2018) stressed the role of \sout{the} the “EuroMaydan” page which was created on November 21, 2013 in order to support the revolution. This page generated more than 600,000 comments, 2.2 million “shares,” and 7.9 million “likes.” Jost et al. (2018) suggest that this page gained informational relevance in the course of the protest using the steady increase of this page as evidence. Also, remarkably, the Twitter activities were typically very low in Ukraine. However, the number of participants of Twitter increased with protest. Which suggests that many Ukrainians were likely to join Twitter to follow the events of the revolution. 
%Although empirical evidence suggests that spikes in online activities corresponded with periods of important offline activities, the causal link between them is very difficult to establish (Little 2016). We will investigate whether individuals who were exposed to the content of the major Facebook page “EuroMaydan” nudged their behavior in line with the agenda of revolution. Previous studies showed that “many people who listed Ukrainian (UK) as their
%preferred language when they registered their Twitter accounts also tweeted in Russian, and many people who listed Russian (RU) as their preferred language also tweeted in Ukrainian” (Jost et al. 2018). This is a typical situation for the Ukrainian public space where people have used both languages consistently for decades (Kulyk 2011). Studies show that people use Ukrainian language themselves and support Ukrainian language in general to signal their Ukrainian identity. Given that EuroMaydan revolution exploited national narratives of Ukrainian unity, Ukrainian language, and Ukrainian independence we expect that people who identified themselves with the cause of the revolution also nudged towards signaling their Ukrainian identity. Thus, we expect to find that people changed their language preferences from Russian to Ukrainian in the course of the OSM activities.


==> What.tex <==
\section{What has changed in their behaviour in social media?}
\label{sec:Language sentiment patterns}
Another important and complementary aspect that helps us understand how the Euromaidan revolution has affected the identity of the people \fixme{what is the meaning of "identity of the people"?}in Ukraine is individuals' sentiment because knowing people's feelings, we can possibly explain some of their actions. \fixme{not very clear to me}

Incorporating this belief in our analysis, we decide to apply text sentiment analysis to investigate how the behaviour of the users was changing through the revolution with respect to their message sentiments in social media.
We start our analysis again by dividing the posts and messages into two main language groups: Ukrainian and Russian. After that, we examine whether the sentiment of comments and posts are different between these two groups. Then, we investigate how the sentiment changed throughout the revolution and how the users' attitude was changing towards particular politicians, political parties and important events during Euromaidan. We call them hot topics, however, they are not strictly related to topic modelling analysis (more details later in this chapter). 
We expect there should be not much difference between the sentiments and attitudes before or in the first months of the revolution, as it was no such obvious intervention of Russia. However, these changes can be more prominent after some significant events, such as the annexation of Crimea, when Ukrainians start to differentiate themselves more from Russia, and one of the consequences switch from Russian to Ukrainian on a daily basis.    

To classify the sentiment of the message, we tried two types of models on our data: a sentiment classification model from a Python package called \textit{polyglot}\footnote{\url{https://pypi.org/project/polyglot/}} and transformer-based neural networks from \textit{HuggingFace}\footnote{\url{https://huggingface.co/}} (each model for each language, 4 in total). To select the best candidate for our analysis, we randomly selected 2000 comments: 1000 comments in Russian and 1000 comments in Ukrainian. Then we manually assign the sentiment of each of the comments in three categories: positive, neutral and negative and run each of the models on them to calculate the accuracy metrics. It turns out that the transformer base models have higher metrics than the model we used from \textit{polyglot} (95\% to 86\%), so we stick to it and, given a relatively high performance for the reliable results, we continue our analysis. 

\subsection{Individuals attitude towards hot topics}
Here we investigate how sentiments towards politicians, political parties, and important events during the Euromaidan revolution (hot topics) vary with respect to Russian and Ukrainian languages of discussions. Firstly, we present a more detailed set of topics for which we calculate the sentiments (topics presented in English): 
\textit{Ukraine}, 
\textit{Russia}, 
\textit{Yanukovych}\footnote{\url{https://en.wikipedia.org/wiki/Viktor_Yanukovych}}, 
\textit{Putin}, 
\textit{European Union}, 
\textit{Fatherland}\footnote{\url{https://en.wikipedia.org/wiki/All-Ukrainian_Union_\%22Fatherland\%22}}, \fixme{Fix link}
\textit{Udar}\footnote{\url{https://en.wikipedia.org/wiki/Ukrainian_Democratic_Alliance_for_Reform}}, 
\textit{Svoboda}\footnote{\url{https://en.wikipedia.org/wiki/Svoboda_(political_party)}}, 
\textit{Azarov}\footnote{\url{https://en.wikipedia.org/wiki/Mykola_Azarov}}, 
\textit{USA}, 
\textit{Poroshenko}\footnote{\url{https://en.wikipedia.org/wiki/Petro_Poroshenko}}, 
\textit{Maidan}, 
\textit{Yatsenyuk}\footnote{\url{https://en.wikipedia.org/wiki/Arseniy_Yatsenyuk}}, 
\textit{Crimea}.

We select the exact set of words based due to several reasons. Firstly, we have some domain knowledge because they are Ukrainians \fixme{Can we write so?}. The second point is that all of these words were one of the most frequently used words in the news, social media, and people shape the revolution in one or another way. We understand that the topics are still subjective, and one can ask why the authors haven't used another political or the name of the political party. Our main motivation is to check if the behaviour has changed in general towards some pro-Russian and pro-Ukrainian political or political parties, but not how the sentiment changed on the individual level.

\fixme{In previous chapters we compared users who spoke primarily in Russian and Ukrainian with respect to how sticky their language choices were. 

There are several reasons for selecting these specific topics. First of all, while the revolution itself was associated with various social and political grievances, most debates gravitated around the issue of political power [ref. Umland]. The role of local and foreign political forces was discussed intensively. With time, the participation of the far-right parties became a salient issue for the international and local media [ref. Ischenko]. Therefore, we selected a list of the political parties which eventually made it to the Parliament, names of most prominent politicians, and words associated with the events of Euromaidan. 
}


 

Now, we briefly explain our sentiment classification procedure for each of the topics, given an already processed two subsets of messages in Russian and Ukrainian languages. 
\begin{enumerate}
    \item Select a language 
    \item Select a word from a proposed set of the hot topics in a given language
     \item For each of the messages in a subset of the messages for a given language:
        \begin{enumerate}
    	    \item Check whether the word in this message or not
    	    \item If the word is in a message, calculate the sentiment of the overall message
    	    \item Otherwise, skip the word and continue.
    	 \end{enumerate}
    \item Finally, give the \texit{average} sentiment of the word based on the message sentiments in which this word appear
\end{enumerate}
Table \ref{table:sentiment_table} shows sentiments taking into account all the dataset for the whole time period. 

\begin{table}[h]
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\textbf{Topic}           & \textbf{Russian} & \textbf{Ukrainian} \\ \hline
\textit{Ukraine}        & Neutral                & Positive                  \\ \hline
\textit{Russia}         & Neutral                & Neutral                  \\ \hline
\textit{USA}            & Neutral                & Neutral                  \\ \hline
\textit{Crimea}         & Neutral                & Neutral                  \\ \hline
\textit{Maidan}         & Neutral                & Positive                  \\ \hline
\textit{Putin}          & Neutral                & Neutral                  \\ \hline
\textit{Yanukovych}     & Neutral                & Neutral                  \\ \hline
\textit{Azarov}         & Neutral                & Neutral                  \\ \hline
\textit{Poroshenko}     & Positive               & Positive                  \\ \hline
\textit{Yatsenyuk}      & Neutral                & Neutral                  \\ \hline
\textit{European Union} & Neutral                & Positive                 \\ \hline
\textit{Fatherland}     & Neutral                & Neutral                 \\ \hline
\textit{Udar}           & Neutral                & Neutral                 \\ \hline
\textit{Svoboda}        & Positive               & Positive                 \\ \hline
\end{tabular}%
}
\caption{Sentiments of the proper names in Russian and Ukrainian comments}
\label{table:sentiment_table}
\end{table}

\subsection{The mood the individuals}
We believe that understanding the sentiment from the angle of attitude towards some specific topics is not enough. To make our analysis more coherent, we also investigate the general mood of people on average and during the different stages of the revolution. The procedure is similar to the previous subsection, but here we are only interested in the sentiment of the message and then calculate either average thought all the comments in a particular message on the whole dataset, or split the dataset into chunks given the time and calculate the sentiment score for each of the chunk.

\subsection{Which language contains more positive messages: Russian or Ukrainian?}
We received that the number of positive messages in the Ukrainian language was higher than in the Russian language. More precisely, the average sentiment of all comments in the Ukrainian language is 0.23 and in Russian is -0.0034. 

\subsection{Which individuals are more positive: Russian or Ukrainian speaking?}
At the same time, we check the average sentiment by the user and the average sentiment of the Ukrainian and Russian comment users. Again, it turns out that the commenters who prefer the Ukrainian language, in general, are more positive than those who mostly use the Russian language.

% \subsection{How the mood was changing thought the revolution timeline?}



